Maya: Falsifying Power Sidechannels with Dynamic Control

The security of computers is at risk because of information leaking through physical outputs such as power, temperature, or electromagnetic (EM) emissions. Attackers can use advanced signal measurement and analysis to recover sensitive data from these sidechannels. To address this problem, this paper presents Maya, a simple and effective solution against power side-channels. The idea is to re-shape the power dissipated by an application in an application-transparent manner using control theory techniques - preventing attackers from learning any information. With control theory, a controller can reliably keep power close to a desired target value even when runtime conditions change unpredictably. Then, by changing these targets intelligently, power can be made to appear in any desired form, appearing to carry activity information which, in reality, is unrelated to the application. Maya can be implemented in privileged software or in simple hardware. In this paper, we implement Maya on two multiprocessor machines using Operating System (OS) threads, and show its effectiveness and ease of deployment.

==> design.tex <==
\section{\des: Protecting Against Power Analysis Attacks }
\label{design}

The security of computers is at risk because of information leaked inadvertently through its physical side channels.  \des is an OS-level defense system that prevents information leakage by changing a computer's power. The key idea in \des is simple --- give the illusion of fake output activity by changing inputs intelligently. With \des, a computer's power measurements still exhibit patterns, but which, are unrelated to the application. Therefore, signal analysis recovers only fake activity. 

 


\subsection{Controller}
\label{sub_robustC}

The Controller finds the input values to keep the outputs close to the targets. It reads the targets from the Mask Generator and the actual output measurements from sensor drivers. We design the controller with MIMO Robust control theory~\cite{mimoText}. The Controller finds the inputs using Equation~\ref{eq:control} and its working is described in Section~\ref{sub_robust}. 

Robust control theory is the enabling technology for \des. Being MIMO, the controller can simultaneously change the multiple inputs in our design to keep all outputs close to their targets. 

 Robust controllers also guarantee that the deviations of outputs from their targets are always kept below designer specified bounds. This is essential for \des to effectively manipulate the information revealed by output analysis. With non-robust control, it is difficult to make the outputs accurately follow their targets. Consequently, the outputs cannot mislead signal analysis. 

The controller's robustness allows \des to work across applications that differ in their activity profile and response to inputs. Non-robust controllers fail to accuractely follow the targets when runtime conditions differ from the information used in its design. In contrast, robust controllers are designed with uncertainty guardbands (Section~\ref{sub_robust}) and can accurately track the targets as long as the runtime response of the system is within the guardband~\cite{mimoText}. Fortunately, these guardbands can be large without slowing the controller~\cite{mimoText}.

\subsection{Elastic Applications}
\label{sub_elastic}

The Elastic applications serve as inputs in addition to DVFS and idle cycle injection (Section~\ref{sub_inputs}). They take in one or more runtime parameters and vary their power consumption from a minimum level (i.e., sleep) to maximum power. 
The elastic applications are pacakged with \des and can interrupt the regular applications.



The elastic applications enable \des overcome three problems. First, there is  a lack of OS level inputs that can reliably change power across a large range. Options like DVFS or idle cycle injection work well in only some cases (Section~\ref{sub_inputs}). Without reliable actuators, a computer's power cannot be changed, leaving it vulnerable to information leakage. The elastic applications address this limitation.

\josep{do not talk about osciloscope}

Second, if DVFS alone is used to change power, attackers can detect the change in the frequency by measuring the computer's EM emissions~\cite{emAttack,genkinEm} or by reading power through a high resolution oscilloscope~\cite{dvfsSecurityEval,randomDvsDfs}. Once the frequency is determined, it is possible to re-scale the power trace. Using the elastic applications apart from DVFS prevents this because power changes can be triggered from multiple inputs now. 

Finally, by working as actuators at the software level, the elastic applications allow \des to be deployed on many existing systems without needing extra hardware support.


\subsection{Deploying \des}
\label{sub_deploy}

\des is intended to be deployed as a part of the OS, requiring administrative privileges to interact with the sensor and input drivers . \des can be considered to be similar to power governors in linux~\cite{linuxGovernors}. \rpp{Therefore, applications can request Maya to be active only when it is necessary to perform security-sensitive operations on their systems. In such cases, Maya will start when \textit{any} application triggers it and stop only after \textit{all} applications issue stop requests.} 

The Mask Generator and Controller run periodically while the Elastic applications run always. These applications are also run with administrative privileges and cannot be modified from user space. 





==> sensitivity.tex <==
\section{Sensitivity to \des Design Parameters}
\label{sensitivity}


\begin{comment}
\subsection{Impact of Sampling Interval}
\label{sub_sampling}

Slow: apply more complex masking patterns, use\# cores too.
Here, there are two options one MIMO or 2 MIMO - one with all fast inputs like frequency, balloons and the other with \# cores etc.

\subsection{Impact of channel leakage}
\label{sub_leakage}

What can attacker know if one of the channels is revealed.
Analysis from model.
\end{comment}
